LVOS: A Benchmark for Long-term Video Object Segmentation

Existing video object segmentation (VOS) benchmarks focus on short-term videos which just last about 3-5 seconds and where objects are visible most of the time. These videos are poorly representative of practical applications, and the absence of long-term datasets restricts further investigation of VOS on the application in realistic scenarios. So, in this paper, we present a new benchmark dataset named \textbf{LVOS}, which consists of 220 videos with a total duration of 421 minutes. To the best of our knowledge, LVOS is the first densely annotated long-term VOS dataset. The videos in our LVOS last 1.59 minutes on average, which is 20 times longer than videos in existing VOS datasets. Each video includes various attributes, especially challenges deriving from the wild, such as long-term reappearing and cross-temporal similar objeccts.Based on LVOS, we assess existing video object segmentation algorithms and propose a Diverse Dynamic Memory network (DDMemory) that consists of three complementary memory banks to exploit temporal information adequately. The experimental results demonstrate the strength and weaknesses of prior methods, pointing promising directions for further study. Data and code are available at https://lingyihongfd.github.io/lvos.github.io/.

==> sections/1_abstract.tex <==
%%%%%%%%% ABSTRACT
\begin{abstract}
   Existing video object segmentation (VOS) benchmarks focus on short-term videos which just last about 3-5 seconds and where objects are visible most of the time. These videos are poorly representative of practical applications, and the absence of long-term datasets restricts further investigation of VOS on the application in realistic scenarios. So, in this paper, we present a new benchmark dataset named \textbf{LVOS}, which consists of 220 videos with a total duration of 421 minutes. To the best of our knowledge, LVOS is the first densely annotated long-term VOS dataset. The videos in our LVOS last 1.59 minutes on average, which is 20 times longer than videos in existing VOS datasets. Each video includes various attributes, especially challenges deriving from the wild, such as long-term reappearing and cross-temporal similar objeccts.
		Based on LVOS, we assess existing video object segmentation algorithms and propose a \textbf{D}iverse \textbf{D}ynamic \textbf{Memory} network (\textbf{DDMemory}) that consists of three complementary memory banks to exploit temporal information adequately. The experiment results demonstrate the strength and weaknesses of prior methods, pointing promising directions for further study. 
		Data and code are available at \url{https://lingyihongfd.github.io/lvos.github.io/}.

==> sections/2_intro.tex <==
%%%%%% table dataset
\begin{table*}
		\setlength{\abovecaptionskip}{2pt}%    
		\setlength{\belowcaptionskip}{0pt}%
        \setlength{\tabcolsep}{1.6mm} 
		\centering
		%\tiny
        %\scriptsize
        \footnotesize
        \input{./tables/static}
        \caption{Comparison of LVOS with the most popular video segmentation and tracking benchmarks. The top part is existing short-term video datasets and the bottom part is long-term video datasets. Duration denotes the total duration (in minutes) of the annotated videos. Annotations type means the type of groundtruth annotations. \textbf{M} and \textbf{B} denote mask and box annotations. \textbf{N} means that the groundtruth annotations are unavailable. The largest value is in bold, and the second and third largest values are underlined.}
		\label{tab:dataset_static}
		\vspace{-6mm} 
\end{table*}
